The Quantum Approximate Optimization Algorithm performance with low entanglement and high circuit depth

Variational quantum algorithms constitute one of the most widespread methods for using current noisy quantum computers. However, it is unknown if these heuristic algorithms provide any quantum-computational speedup, although we cannot simulate them classically for intermediate sizes. Since entanglement lies at the core of quantum computing power, we investigate its role in these heuristic methods for solving optimization problems. In particular, we use matrix product states to simulate the quantum approximate optimization algorithm with reduced bond dimensions $D$, a parameter bounding the system entanglement. Moreover, we restrict the simulation further by deterministically sampling solutions. We conclude that entanglement plays a minor role in the MaxCut and Exact Cover 3 problems studied here since the simulated algorithm analysis, with up to $60$ qubits and $p=100$ algorithm layers, shows that it provides solutions for bond dimension $D \approx 10$ and depth $p \approx 30$. Additionally, we study the classical optimization loop in the approximated algorithm simulation with $12$ qubits and depth up to $p=4$ and show that the approximated optimal parameters with low entanglement approach the exact ones.

==> Figures/PRDMmps1.tex <==
\begin{tikzpicture}
    
    % first row
    \node[block, thick] (a) {$A^{\dagger s_1}$};
        \node[circle,draw,thick,below of=a] (a1) {};
            \node[circle,draw,thick,below of=a1] (a11) {};
                \node[block, thick, below of=a11] (A) {$A^{s_1}$};
            
    \node[block, thick, right of=a, xshift=.25cm] (b) {$A^{\dagger s_2}$};
        \node[rectangle,draw,thick,below of=b,minimum size = 0.29cm] (b1) {};
            \node[rectangle,draw,thick,below of=b1,minimum size = 0.29cm] (b11) {};
                \node[block, thick, below of=b11] (B) {$A^{s_2}$};
            
    \node[block, thick, right of=b, xshift=.25cm] (c) {$A^{\dagger s_3}$};
        \node[circle,draw,thick,below of=c] (c1) {};
            \node[circle,draw,thick,below of=c1] (c11) {};
                \node[block, thick, below of=c11] (C) {$A^{s_3}$};
            
    \node[right of=c, xshift=.25cm] (d) {$\dots$};
    \node[right of=C, xshift=.25cm] (D) {$\dots$};
    
    % \node[right of=b, xshift=.25cm] (d) {$\dots$};
    % \node[right of=B, xshift=.25cm] (D) {$\dots$};
    
    \node[block, thick, right of=d, xshift=.25cm] (e) {$A^{\dagger s_k}$};
        \node[below of=e] (e1) {};
            \node[below of=e1] (e11) {};
                \node[block, thick, below of=e11] (E) {$A^{s_k}$};
            
    \node[right of=e, xshift=.25cm] (f) {$\dots$};
    \node[right of=E, xshift=.25cm] (F) {$\dots$};
    
    % \node[block, thick, right of=f, xshift=.25cm] (g) {$A^{\dagger s_{N\text{-}1}}$};
    %     \node[below of=g] (g1) {};
    %         \node[below of=g1] (g11) {};
    %             \node[block, thick, below of=g11] (G) {$A^{s_{N\text{-}1}}$};
            
    \node[block, thick, right of=f, xshift=.25cm] (h) {$A^{\dagger s_n}$};
        \node[below of=h] (h1) {};
            \node[below of=h1] (h11) {};
                \node[block, thick, below of=h11] (H) {$A^{s_n}$};;
            
    % \node[right of=h, xshift=.25cm,yshift=-0.475cm] (i) {};
    %     \node[below of=i] (i1) {$=$};
    %         \node[below of=i1] (I) {};;
            
    % \node[right of=i, xshift=.25cm] (j) {};
    %     \node[block, thick, below of=j] (j1) {$\rho^{k}$};
    %         \node[below of=j1] (J) {};;
            
    % \draw[black,very thick] (j) -- (j1);
    % \draw[black,very thick] (j1) -- (J);
    
    \node[below of=D] (i) {$\Downarrow$};

    \node[block, thick, below of=i] (j) {$\rho^{k}$};
        \node[right of=j] (jr) {};
            \node[left of=j] (jl) {};
        
    \draw[black,very thick] (j) -- (jr);
    \draw[black,very thick] (jl) -- (j);
            
    
    % \draw[black,very thick] (a) -- (b) -- (d) -- (e) -- (f) -- (g) -- (h);
    % \draw[black,very thick] (A) -- (B) -- (D) -- (E) -- (F) -- (G) -- (H);
    
    \draw[black,very thick] (a) -- (b) -- (c) -- (d) -- (e) -- (f) -- (h);
    \draw[black,very thick] (A) -- (B) -- (C) -- (D) -- (E) -- (F) -- (H);
    
    % \draw[black,very thick] (a) -- (b) node [midway] {$u_1$};
    % \draw[black,very thick] (b) -- (c) {$u_2$};
    % \draw[black,very thick] (c) -- (d) {$u_3$};
    % \draw[black,very thick] (d) -- (e) {$u_{k-1}$};
    % \draw[black,very thick] (e) -- (f) {$u_k$};
    % \draw[black,very thick] (f) -- (g) {$u_{N-1}$};
    % \draw[black,very thick] (g) -- (h) {$u_n$};
    % \draw[black,very thick] (a) -- (A);
    % \draw[black,very thick] (b) -- (B);
    % % \draw[black,very thick] (c) -- (C);
    % \draw[black,very thick] (g) -- (G);
    % \draw[black,very thick] (h) -- (H);
    % \draw[black,very thick] (e) -- (e1);
    % \draw[black,very thick] (e11) -- (E);
    
    
    \draw[black,very thick] (a) -- (a1);
    \draw[black,very thick] (a11) -- (A);
    \draw[black,very thick] (b) -- (b1);
    \draw[black,very thick] (b11) -- (B);
    \draw[black,very thick] (c) -- (c1);
    \draw[black,very thick] (c11) -- (C);

    \draw[black,very thick] (e) -- (e1);
    \draw[black,very thick] (e11) -- (E);
    
    \draw[black,very thick] (h) -- (H);

    
\end{tikzpicture}   

==> Figures/qaoa.tex <==
            \begin{adjustbox}{width=0.8\textwidth}
              \begin{quantikz}[row sep=2mm,column sep=3mm,scale=.2]
                % First row
                \lstick[wires=4]{$\ket{0}^{\otimes n}$}
                & \gate[style={fill=pink!60}]{H}                                        % 1
                & \gate[4,nwires={3},style={fill=yellow!30}]{e^{-i\gamma_1\hat{H}_C}}     % 2
                \gategroup[wires=4,steps=2,
                  style={dashed,rounded corners,fill=blue!20,inner sep=2pt},
                  background]
                {$p=1$}
                & \gate[style={fill=green!20}]{R_x(2\beta_1)}                           % 3
                & \ \ldots\ \qw                                                         % 4
                & \gate[4,nwires={3},style={fill=yellow!30}]{e^{-i\gamma_P\hat{H}_C}}     % 5
                \gategroup[wires=4,steps=2,
                  style={dashed,rounded corners,fill=blue!20,inner sep=2pt},
                  background]
                {$p=P$}
                & \gate[style={fill=green!20}]{R_x(2\beta_P)}                           % 6
                & [2mm] \meter[fill=orange!80]{}                                        % 7
                & \cw                                                                   % 8
                & \gate[4,
                  nwires={3},
                  cwires={1,2,4},
                  disable auto height,
                  style={fill=red!30},
                  label style={rotate=0}]{
                  \begin{array}{c}
                    \textbf{Optimize} \\
                    \langle\vec{\gamma},\vec{\beta}|\hat{H}_C|\vec{\gamma},\vec{\beta}\rangle
                  \end{array}}                                                          % 9
                \\
                % Second row
                & \gate[style={fill=pink!60}]{H}                                        % 1
                &                                                                       % 2
                & \gate[style={fill=green!20}]{R_x(2\beta_1)}                           % 3
                & \ \ldots\ \qw                                                         % 4
                &                                                                       % 5
                & \gate[style={fill=green!20}]{R_x(2\beta_P)}                           % 6
                & [2mm] \meter[fill=orange!80]{}                                        % 7
                & \cw                                                                   % 8
                &                                                                       % 9
                \\
                % Third row
                & \vdots                                                                % 1
                &                                                                       % 2
                & \vdots                                                                % 3
                &                                                                       % 4
                &                                                                       % 5
                & \vdots                                                                % 6
                & \vdots                                                                % 7
                &                                                                       % 8
                &                                                                       % 9
                \\
                % Fourth row
                & \gate[style={fill=pink!60}]{H}                                        % 1
                &                                                                       % 2
                & \gate[style={fill=green!20}]{R_x(2\beta_1)}                           % 3
                & \ \ldots\ \qw                                                         % 4
                &                                                                       % 5
                & \gate[style={fill=green!20}]{R_x(2\beta_P)}                           % 6
                &[2mm] \meter[fill=orange!80]{}                                         % 7
                & \cw                                                                   % 8
                &                                                                       % 9
                \\[2em]
                % Fifth row
                &                                                                       % 1
                &\gategroup[wires=1,
                  steps=5,
                  style={fill=red!30,inner sep=5pt,rounded corners},
                  label style={label position=center,anchor=north,yshift=-.2cm}]
                {Update variational parameters $(\vec{\gamma},\vec{\beta})$}
                \arrow[u]
                %\arrow[u,shift right=4cm,yshift=-2mm]                                  % 2
                &\arrow[u]                                                              % 3
                &                                                                       % 4
                &\arrow[u]                                                              % 5
                &\arrow[u]                                                              % 6
                &\cw                                                                    % 7
                &\cw                                                                    % 8
                &\cwbend{-1}                                                            % 9
                \\
                % Sixth Row
                &                                                                       % 1
                &                                                                       % 2
                &                                                                       % 3
                &                                                                       % 4
                &                                                                       % 5
                &                                                                       % 6
                &                                                                       % 7
                &                                                                       % 8
                &                                                                       % 9
              \end{quantikz}
            \end{adjustbox}
            
